Parallel Backpropagation for Inverse of a Convolution with Application to Normalizing Flows

The inverse of an invertible convolution is an important operation that comes up in Normalizing Flows, Image Deblurring, etc. The naive algorithm for backpropagation of this operation using Gaussian elimination has running time $O(n^3)$ where $n$ is the number of pixels in the image. We give a fast parallel backpropagation algorithm with running time $O(\sqrt{n})$ for a square image and provide a GPU implementation of the same. Inverse of Convolutions are usually used in Normalizing Flows in the sampling pass, making them slow. We propose to use the Inverse of Convolutions in the forward (image to latent vector) pass of the Normalizing flow. Since the sampling pass is the inverse of the forward pass, it will use convolutions only, resulting in efficient sampling times. We use our parallel backpropagation algorithm to optimize the inverse of the convolution layer, resulting in fast training times. We implement this approach in various Normalizing Flow backbones, resulting in our Inverse-Flow models. We benchmark Inverse-Flow on standard datasets and show significantly improved sampling times with similar bits per dimension compared to previous models.

==> sections/inv_conv.tex <==
\section{Backpropagation algorithm for Inverse of Convolution}

\subsection{Notation and Setup}

Let us denote the input to the inverse of convolution (inv-conv) by $y \in \mathbb{R}^{m^2}$ and the output by $x \in \mathbb{R}^{m^2}$. We index $x$ and $y$ using $p = (p_1, p_2) \in \{1, \ldots, n\} \times \{1, \ldots, n\}$. We define:

\begin{equation}
    \Delta(p) = \{(i,j) : 0 \leq p_1 - i, p_2 - j < k\} \setminus \{p\}
\end{equation}

$\Delta(p)$ represents the set of all pixels, except $p$, which depend on $p$ when convolution is applied with top and left padding. We also define a partial ordering $\leq$ on pixels as follows:

\begin{equation}
    p \leq q \quad \Leftrightarrow \quad p_1 \leq q_1 \text{ and } p_2 \leq q_2
\end{equation}

The kernel of the $k \times k$ convolution is given by the matrix $W \in \mathbb{R}^{k \times k}$.

\subsection{Theorem Statement}

\begin{theorem}
For the inverse convolution operation, the partial derivative of the output with respect to the input is given by:

\begin{equation}
    \frac{\partial x_q}{\partial y_p} = 
    \begin{cases}
        1 & \text{if } p = q \\
        0 & \text{if } q \not\leq p \\
        -\sum_{r \in \Delta(p)} W_{(k,k) - r} \frac{\partial x_{p-r'}}{\partial y_p} & \text{otherwise}
    \end{cases}
\end{equation}
\end{theorem}

\subsection{Theorem Explanation}

The theorem present computing $\frac{\partial x_q}{\partial y_p}$, which represents how a change in the input pixel $y_p$ affects the output pixel $x_q$ in an inverse of convolution operation. Let's break down each case:

\emph{Case 1: $p = q$}\\

When $p = q$, we have:

\begin{equation}
    \frac{\partial x_q}{\partial y_p} = 1
\end{equation}

This case represents the direct influence of an input pixel on its corresponding output pixel. The derivative is 1, indicating a one-to-one relationship.

\emph{Case 2: $q \not\leq p$}\\

When $q \not\leq p$, we have:

\begin{equation}
    \frac{\partial x_q}{\partial y_p} = 0
\end{equation}

This case uses the partial ordering defined earlier. If $q$ is not less than or equal to $p$ in this ordering, it means that the output pixel $x_q$ is not influenced by the input pixel $y_p$ in the inverse convolution operation. Therefore, the derivative is 0.

\emph{Case 3: Otherwise}\\

For all other cases:

\begin{equation}
    \frac{\partial x_q}{\partial y_p} = -\sum_{r \in \Delta(p)} W_{(k,k) - r} \frac{\partial x_{p-r'}}{\partial y_p}
\end{equation}

This case is more complex:

\begin{itemize}
    \item $\Delta(p)$ is the set of all pixels (except $p$) that depend on $p$ in a regular convolution operation.
    \item $W_{(k,k) - r}$ represents the weight in the convolution kernel corresponding to the relative position of $r$.
    \item $\frac{\partial x_{p-r'}}{\partial y_p}$ is a recursive term, representing how changes in $y_p$ affect $x$ at a different position.
\end{itemize}

The negative sign and the summation in this formula account for the inverse nature of the operation and the cumulative effects of the convolution kernel.

\paragraph{Significance and Application}

This theorem is crucial for computing the gradients in the backpropagation algorithm for inverse convolution layers. By providing a way to calculate $\frac{\partial x_q}{\partial y_p}$, it allows us to compute $\frac{\partial L}{\partial y_p}$ using the chain rule:

\begin{equation}
    \frac{\partial L}{\partial y_p} = \sum_{q} \frac{\partial L}{\partial x_q} \times \frac{\partial x_q}{\partial y_p}
\end{equation}

Where $L$ is the loss function. This, in turn, enables the optimization of inverse of convolution layers in neural networks using gradient-based methods.

\paragraph{Conclusion}

Understanding and implementing this theorem is fundamental to the efficient computation of gradients in inverse convolution layers. It provides a structured approach to calculating the necessary partial derivatives, taking into account the complex relationships between input and output pixels in the inverse convolution operation. This theorem forms the basis for implementing backpropagation in neural networks that utilize inverse convolution layers, allowing for their effective training and optimization.

==> sections/trash.tex <==
%% Formal proof: Theorem 1



%% intro

% %Tips:  what not how 
% % \item Training of proposed Inverse-Flow model and extensive sampling time comparison.

%https://proceedings.neurips.cc/paper_files/paper/2019/file/b1f62fa99de9f27a048344d55c5ef7a6-Paper.pdf
% Normalizing Flow models map complex data distribution of training set to a simple data distribution (e.g., Normal distribution) and then generate new and unknown samples from mapped distribution.  It has recently been shown that invertible networks can be designed and can still be trained to perform discriminative tasks successfully. These networks hold promise for more direct feature visualization, low memory training, and designing expressive normalizing flows. Transformation of convolution function (bijective function) to define a normalized density requires computation of a Jacobian determinant, which is generally impractical for arbitrary neural network transformations. To overcome this difficulty and enable fast computation, previous works \citep{kingma2018glow, karami2019invertible, hoogeboom2019emerging,  nagar2021cinc, visapp23} have carefully designed architectures that produce simple and Jacobian forms.

% With other models such as Diffusion \citep{dhariwal2021diffusion, rombach2022high}, GANs \citep{brock2018large, zhang2019self}: invert-ability is ill-posed and based on assumption and approximation. However, with exact inverse, freedom of latent vector to generate out-of-distribution samples and latent space exploration can be achieved with normalizing flow models \citep{rezende2015variational}. The bottleneck for normalizing flow depends on invertibility speed and same dimension for entire computation cost of network \citep{papamakarios2021normalizing}. This restricts flow models to slow sampling and invertibility of convolution.  We propose a new invertible convolution ($f$) with a trainable inverse ($f^{-1}$) using a backpropagation algorithm for inverse of $f$. Inverse-flow, Normalizing flow models maintain strong inductive biases that Convolutional networks possess for discriminative tasks. We proposed a backpropagation algorithm for inverse of invertible convolution with parallelization on GPUs using CUDA implementation.

% Specifically, we show how convolutions can be converted into crude normalizing flow models with training inverse of convolution ($f$) in forward pass and convolution ($f^{-1}$) to generate samples. We developed backpropagation algorithm for inverse of convolutions, trained flow (sequence of inverse convolution layers), and learned mapping of data distribution to normal distribution ($N(0, I)$). Because procedure can be applied to high performance of existing CNN architectures, we can hope to design invertible neural networks useful for both generative and discriminative modelling.

% \paragraph{Our contributions.} In this work, we propose a flow model, \emph{Inverse-Flow}, using inverse of invertible convolution ($f^{-1}$) in forward pass and invertible convolution ($f$) for data generation. Inverse-flow models generate faster samples than standard flow modes. We provide an implementation of Inverse-Flow (together with baselines and experiments) in C++ at a publicly available repository \footnote{\url{https://github.com/Naagar/Inverse-Flow}}. The code is parallelized via Ninja and Cython framework and comes with a Python interface. In summary, our contribution includes:
% \begin{enumerate}
%     \item Fast Invertible Convolution ($inv\_conv$) layers with trainable inverse for Normalizing Flow.
%     \item Multi-scale Inverse Flow Architecture for Fast sampling Flow model.
%     \item Fast and parallelized backpropagation algorithm  for $inv\_conv^{-1}$ using independence of $inv\_conv$ operations. 
%     \item GPU (CUDA) implementation of proposed Inverse-Flow and Backpropagation Algorithm. 

%     \item Training of proposed Inverse-Flow model and extensive sampling time comparison.
% \end{enumerate}




% Convolutional neural networks (ConvNets)(LeCun et al., 1990) have proved incredibly effective for problems with translational structure and spatial locality.


% inv_bpp


% inverse_flow

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TRASH
%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Complexity of Jacobian for Invertible Convolutions}
% A key challenge in designing efficient normalizing flows is managing the computational complexity of the Jacobian determinant. For invertible convolutions, which are a popular choice for constructing flexible normalizing flows, the complexity of computing the Jacobian determinant is of particular interest.


% Consider an invertible convolution operation on a 3D tensor of shape $(C, H, W)$, where $C$ is the number of channels, and $H$ and $W$ are the spatial dimensions. The weight matrix $\mathbf{W}$ for this operation has dimensions $C \times C$.

% The Jacobian of this transformation is a block-circular matrix, where each block is of size $C \times C$, and there are $H \cdot W$ blocks. Naively computing the determinant of this matrix would have a complexity of $\mathcal{O}((CHW)^3)$, which is prohibitively expensive for most practical applications.

% However, we can significantly reduce this complexity by leveraging the properties of block-circular matrices and the convolution operation. The determinant of the Jacobian can be computed as:

% \begin{equation}
% \det\left(\frac{\partial f}{\partial \mathbf{z}}\right) = \prod_{i=1}^{H} \prod_{j=1}^{W} \det(\hat{\mathbf{W}}_{ij})
% \end{equation}

% where $\hat{\mathbf{W}}_{ij}$ are the eigenvalues of $\mathbf{W}$ in the Fourier domain. This reduces the complexity to $\mathcal{O}(C^3 + CHW\log(HW))$, where:

% \begin{itemize}
%     \item $\mathcal{O}(C^3)$ comes from computing the determinant of the $C \times C$ weight matrix
%     \item $\mathcal{O}(CHW\log(HW))$ comes from the Fast Fourier Transform (FFT) operations
% \end{itemize}

% This significant reduction in computational complexity makes invertible convolutions a practical choice for constructing expressive normalizing flows, especially for high-dimensional data such as images.

% In our approach, we utilize invertible convolutions ($inv\_conv$) with efficient Jacobian computation to $O(nk^2)$ with parallelized for carefully designed convolutions \cite{visapp23}.


%% results

%% Todo: images diff and recon for all models in one picture






% \begin{table}[t]
%     \centering
%         \begin{tabular}{ccc}
%         \toprule
%         \textbf{Method} & \textbf{Sampling (sec)} & \textbf{BPD} \\
%         \midrule
%         Inverse-Flow (our) & 96.24 & 3.02 \\
%         SNF            & 199.0 & 3.37 \\
%         % FIncFlow       & Dataset 3 & 90.2\% & 15.6 \\
%         % MaCow          & Dataset 3 & 90.2\% & 15.6 \\
%         % Butterfly Flow & Dataset 3 & 90.2\% & 15.6 \\
%         \bottomrule
%         \end{tabular}
%     \caption{Performance comparison of different methods for the CIFAR10 dataset with block size (K) = 4 and number of blocks(L) = 2.}
%     \label{tab:C_st_2_4}
% \end{table}

% Inverse-Flow Conv. 9-Layer (our)        & 20.2 $\pm 0.2$ & 105 $\pm 2.3$  & 0.0957 \\
        % \hline 
        % Glow 2L-16K               & 575.7 $\pm 0.8$ & 20.01 $\pm 2.6$ & 206 $\pm 5.1$ & 0.5536 \\
        % SNF 2L-16K                & 575.4 $\pm 1.8$ &  15.07 $\pm 0.6$ & 221 $\pm 1.8$ & 0.5551 \\
        % FInCFlow 2L-16K           & 645.5 $\pm 3.6$ & 104.01 $\pm 1.3$ & 420 $\pm 5.1$ & 0.8273 \\
        % MintNet 2L-16K            & 645.5 $\pm 3.6$ & -- & 320 $\pm 4.3$ & 0.9237 \\
        % Inverse-Flow 2L-16K (our) & 578.5 $\pm 1.6$ & 67.13  $\pm 1.3$ & 280 $\pm 3.1$ & 0.9237 \\
        % \hline
        
        % Butterfly Flow & Dataset 3 & 90.2\% & 15.6 \\
        % Exact Conv. 9-Layer Conv. Exponential 9-Layer


% Given: input image $x_{m, m}$ with padding \citep{nagar2021cinc}, kernel $W_{k,k}$ with $m=input\_size$ and $k = kernel\_size$ ($k << n$).\\

% Proposition: Let $y = inv\_conv(x, W)$ (\ref{eq_1}) be an invertible convolution (with Top-Left padding) on input $x$ and $inv\_conv()$ as a bijective function then:\\
% \begin{equation}
%     \includegraphics[width=0.99\linewidth]{images/qe_dy_dw.png}
% \end{equation}

% \begin{equation}
%     \includegraphics[width=1\linewidth]{images/equation_1.pdf}
%     \label{eq_1}
% \end{equation}

% \begin{equation}
%     % \tiny
%     % \small
%     \scriptsize
%     \begin{bmatrix}
%         y_{1,1} & y_{1,2} & y_{1,3} \\
%         y_{2,1} & y_{2,2} & y_{2,3}\\
%         y_{3,1} & y_{3,2} & y_{3,3}\\
%     \end{bmatrix} =   \newline \\
%      \begin{bmatrix}
%         0 & 0       & 0       & 0 \\
%         0 & x_{1,1} & x_{1,2} & x_{1,3} \\
%         0 & x_{2,1} & x_{2,2} & x_{2,3} \\
%         0 & x_{3,1} & x_{3,2} & y_{3,3}
%         \end{bmatrix}
%         *
%         \begin{bmatrix}
%             W_{1,1} & W_{1,2}  \\
%             W_{2,1} & W_{2,2}  \\
%         \end{bmatrix}
%     \label{eq_1}
% \end{equation}

% a). The invertible convolution operation can be expressed as a vector-matrix multiplication $y = M * x$ (\ref{eq_2}) where $M_{m^{2},m^{2}}$ ($m\times m$ = $n$, input size) is a lower half triangular matrix formed by linear transform of $W$. This step consists of transforming convolution operation to matrix multiplication. Therefore, each local window is unrolled into a vector, and then all local windows are grouped in a single matrix.\\
% \begin


% \begin{center}
% \fbox{\parbox{0.5\textwidth}{
% \textbf{Algorithm:} Gradients w.r.t Weights
% \textbf{Input:} $x \in \mathbb{R}^{m \times m}, \frac{\partial L}{\partial y} \in \mathbb{R}^{m \times m}, k \in \mathbb{N}$
% \textbf{Output:} $\frac{\partial L}{\partial W} \in \mathbb{R}^{k \times k}$
% \begin{enumerate}
% \item Initialize $\frac{\partial L}{\partial W} \leftarrow \mathbf{0}_{k \times k}$
% \item For $i = 1$ to $k \times k$:
%     \begin{enumerate}
%     \item For $j = 1$ to $k \times k$:
%         \item For $p_1 = 1$ to $m$:
%             \begin{enumerate}
%             \item For $p_2 = 1$ to $m$:
%                 \item If $1 \leq p_1-(k-i) \leq m$ and $1 \leq p_2-(k-j) \leq m$:            
%                     \item $\frac{\partial L}{\partial W_{ij}} \leftarrow \frac{\partial L}{\partial W_{ij}} + \frac{\partial L}{\partial y_{p_1,p_2}} \cdot x_{p_1-(k-i),p_2-(k-j)}$        
%             \end{enumerate}
%     \end{enumerate}
% \end{enumerate}
% \item Return $\frac{\partial L}{\partial W}$
% }}
% \end{center}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\linewidth]{images/equation_04.pdf}
%     \caption{$y = M * x$.}
%     \label{fig:eq_4}
% \end{figure}

% b). Inverse of convolution (\ref{eq_1}) can be calculated as $x = M^{-1} * y$ as in (\ref{eq-inv}) and can be more simplified as (\ref{eq-xp}).\\
% \begin{equation}
%     \label{eq-inv-copy}
%     % \tiny
%     \begin{bmatrix}
%         x_{1,1} \\
%         x_{1,2} \\
%         x_{1,3} \\
%         x_{2,1} \\
%         x_{2,2} \\
%         x_{2,3} \\
%         x_{3,1} \\
%         x_{3,2} \\
%         x_{3,3} \\
%     \end{bmatrix} 
%     =
%     M^{-1}
%     *
%     \begin{bmatrix}
%         y_{1,1} \\
%         y_{1,2} \\
%         y_{1,3} \\
%         y_{2,1} \\
%         y_{2,2} \\
%         y_{2,3} \\
%         y_{3,1} \\
%         y_{3,2} \\
%         y_{3,3} 
%     \end{bmatrix}
% \end{equation}

% From \ref{eq-yp}, we can get $x_{i, j}$ by following dependency on $x_{i-1, j}, x_{i, j-1}, x_{i-1, j-1} ...$ with $p = (i , j)$ pixel location for $x$. 
% \begin{theorem}
%    \ref{eq-inv} can be written as (\ref{eq-xp}) (cross-correlation operation):
% \begin{equation}
%     \label{eq-xp-copy}
%     x_p = y_p - \sum_{q' \in (0,0) - (k-1,k-1), q' != (0,0) }{W_{(q'- p)} * x_{q'}}
% \end{equation} 

% where $p, q \in {\{0, 1,. . . , m-1\}} * {\{0, 1,. . . , m-1\}}$ p, q denote pixels  and $ p \geq q $ if  $ p_1 \geq q_1 $ $\&$ $ p_2 \geq q_2$.\\ 
% \end{theorem}


% c). In forward pass of Inverse-Flow, we use inverse of invertible convolution (see \ref{eq-inv}) for training and designing backpropagation algorithm for inverse of invertible convolution (see section-\ref{bpa_invCNN}).
% \begin{flalign}
%     \includegraphics[width=0.99\textwidth, left]{images/eq_dy_dw.pdf}
% \end{flalign}
% d). For backward pass (sampling), we use invertible convolution (\ref{eq_3}). \\

% \begin{equation}
%     \label{eq_3}
%     \includegraphics[width=0.99\linewidth]{images/eq_3.png}
% \end{equation}

% \begin{equation}
%     \scriptsize
%     \label{eq_3}
%     \begin{bmatrix}
%         x_{1,1} & x_{1,2} & x_{1,3} \\
%         x_{2,1} & x_{2,2} & x_{2,3}\\
%         x_{3,1} & x_{3,2} & x_{3,3}\\
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%         0 & 0       & 0       & 0 \\
%         0 & y_{1,1} & y_{1,2} & y_{1,3} \\
%         0 & y_{2,1} & y_{2,2} & y_{2,3} \\
%         0 & x_{3,1} & y_{3,2} & y_{3,3}
%     \end{bmatrix}
%     *
%     \begin{bmatrix}
%         W_{1,1} & W_{1,2}  \\
%         W_{2,1} & W_{2,2}  \\
%     \end{bmatrix}
% \end{equation}

% e). We apply masking on the W ($W_{k-1,k-1} =1 $) such that all the diagonal entries of  $M$ ($= (M^{-1})^{-1}$) will be $1$ (see \ref{eq_2}, $w_{k-1,k-1} = 1$).

% f). On other hand, log determinant Jacobian also acts as a log barrier in objective function that, in turn, prevents $M$ from becoming zero, hence enforcing invertibility of the convolution filter.

% g). The invertible convolution, its inverse, and Jacobian determinant can all be efficiently computed in $O(nk^2)$ time. For approximation Flow models, SNF \citep{keller2021self}, time complexity is $O (n^2)$. Our proposed method is $n$  times faster than SOTA, considering $k$ kernel size is small compared to input size $n$ ($\#$ pixels). Invertible inverse convolution ( $inv\_conv$ and $inv\_conv^{-1}$) does not compromise receptive field (RF) of a convolution, which is defined as region in input space that a particular CNN’s feature is looking at.


% Linear translation of invertible convolution layer, mathematical form of this operation looks like this

% \subsection{Back-propagation Algorithm for convolution layer}\label{bpa_cnn}

% % Let’s use chain rule for convolutional layer

% \begin{equation}
%     \frac{\delta{ L}}{ \delta {x}} = Conv. ( \frac{\delta{L} }{\delta{y}}, W^{T}), with-padding.
% \end{equation}

% \begin{equation}
%     \frac{\delta{ L}}{ \delta {W}} = Conv. ( x,  \frac{\delta{L} }{\delta{y}}), without-padding.
% \end{equation}

% Let the output of the convolutional layer be:


% \begin{equation}
%     y = W * x
% \end{equation}

% where: \( W \) is filter (or weight matrix). \( x \) is input. \( * \) represents convolution operation, and \( y \) is output before applying any activation function or bias.


% Assume we have a loss function \( L \), and we want to compute the gradients of the loss with respect to weights \( W \) and input \( x \).

% \paragraph{Step 1: Gradient of Loss with respect to Output}
% Given  loss \( L \), we assume that gradient of loss with respect to output \( y \) is known: $\frac{\partial L}{\partial y}$.


% \paragraph{Step 2: Gradient of Loss with respect to Weights}

% To compute the gradient of the loss with respect tohe filter weights \( W \), we apply the chain rule:

% \begin{equation}
%     \frac{\partial L}{\partial W} = \frac{\partial L}{y} * x
% \end{equation}


% where: \( \frac{\partial L}{\partial y} \) is the gradient of the loss with respect to the output \( y \) and convolution operation is applied between \( \frac{\partial L}{\partial y} \) and the input \( x \).


% \paragraph{Step 3: Gradient of Loss with respect to Input}

% To compute the gradient of the loss with respect to the input \( x \), we use the chain rule again:


% \begin{equation}
%     \frac{\partial L}{\partial x} = W [origin=c]{180} * \frac{\partial L}{\partial y}
% \end{equation}

% where $[origin=c]{180}* $ denotes the convolution with the flipped filter $W$ (rotated by 180 degrees).

% \paragraph{Summary of Gradients}

% \begin{equation}
%     \frac{\partial L}{\partial W} = \frac{\partial L}{\partial y} * x
% \end{equation}


% \begin{equation}
%     \frac{\partial L}{\partial x} = W[origin=c]{180} *  \frac{\partial L}{\partial y}
% \end{equation}


% \subsection{Backpropagation algorithm for inverse of invertible convolution} \label{bpa_invCNN}

 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5555 TRASH TRASH TRASH TRASH $$ %%%%%%%%%%%%%%%%%%%%%%%%%%%555555555555555555

% Linear $1 \times 1$ convolutions layers were designed to increase the effectiveness of coupling layers when paired together. Specifically, they learn a more general partitioning of the input than the naive splitting as done in conventional coupling layers \citep{kingma2018glow}. To compute the Jacobian determinant of $1 \times 1$ convolutions layer, they used the LU decomposition and parameterized $\textbf{W}$ as: 
% \begin{align}
%     \textbf{W} = \textbf{PL} (\textbf{U} + diag(s))
% \end{align}

% where $\textbf{P}$ is a pre-specified orthogonal matrix, $\textbf{L}$ is a lower triangular matrix with ones on the diagonal, $\textbf{U}$ is an upper triangular matrix with zeros on the diagonal, and $s$ is a $c$-dimensional vector. This particular structure in the matrix decomposition allows for the Jacobian determinant to be computed in $O(c)$ rather than $O(c^3)$. Emerging convolution \citep{hoogeboom2019emerging} $O(2n^2k^2)$ and the Woodbury transformation \citep{lu2020woodbury} $O(cn^2)$, leverage similar types of matrix structures such as sparsity to improve the performance of coupling layers without sacrificing efficiency. CInC Flow \citep{nagar2021cinc} introduced $3 \times 3$ invertible convolution with $O(n^2k^2)$ computation and  FInC Flow \citep{visapp23} utilize the independence in the $3 \times 3$ invertible convolution and achieve $O((2n-1)k^2)$ fast compute for the inverse.

% \section{Invertible Convolution layer} 
% Coupling layers \cite{kingma2018glow} are powerful invertible non-linear layers. Coupling layers split the input ($x$) into two parts $x_1$ and $x_2$. Then applies the identity map to $x_1$ and transforms $x_2$ using a learnable affine transformation (with shift
% and scale parameters $s_\theta$ and $b_\theta$) that depends on $x_1$. The
% output of this layer $y$ is obtained by concatenating these two intermediate quantities:
% \begin{align*}
%     % \centering
%     z_1 = x_1; z_2 = x_2 \odot s_{\theta}(x_1) + b_{\theta}(x_1)\\
%     y = concat(z_1, z_2) \hspace{2cm}
% \end{align*}
% Due to its simplicity and efficiency, the coupling layer has become a fundamental building block for most state-of-the-art flow model architectures \citep{ho2019flow++}. However, their effectiveness depends heavily on how the input x is partitioned. Recent works have shown that linear layers can learn an improved partitioning scheme, thereby boosting the performance of downstream coupling layers when used together \citep{kingma2018glow}. 

% \begin{equation}
%     \label{eq-1}
%     % \tiny
%     \begin{bmatrix}
%         y_{1,1} & y_{1,2} & y_{1,3} \\
%         y_{2,1} & y_{2,2} & y_{2,3}\\
%         y_{3,1} & y_{3,2} & y_{3,3}\\
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%     0 & 0       & 0       & 0 \\
%     0 & x_{1,1} & x_{1,2} & x_{1,3} \\
%     0 & x_{2,1} & x_{2,2} & x_{2,3} \\
%     0 & x_{3,1} & x_{3,2} & y_{3,3}
%     \end{bmatrix}
%     *
%     \begin{bmatrix}
%         W_{1,1} & W_{1,2}  \\
%         W_{2,1} & W_{2,2}  \\
%     \end{bmatrix}
% \end{equation}
% {equation}
%     \label{eq-4}
%     % \scriptscriptstyle{
%     % \tiny
%     \begin{bmatrix}
%         y_{1,1} \\
%         y_{1,2} \\
%         y_{1,3} \\
%         y_{2,1} \\
%         y_{2,2} \\
%         y_{2,3} \\
%         y_{3,1} \\
%         y_{3,2} \\
%         y_{3,3} \\
%     \end{bmatrix} 
%     =
%     \begin{bmatrix}
%         W_{2,2} &       0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
%         W_{2,1} & W_{2,2} & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
%         0       & W_{2,1} & W_{2,2} & 0 & 0 & 0 & 0 & 0 & 0  \\
%         0       & W_{1,2} & 0 & W_{2,2} & 0 & 0 & 0 & 0 & 0  \\
%         W_{1,1} & W_{1,2} & 0 & W_{2,1} & W_{2,2} & 0 & 0 & 0 & 0  \\
%         0       & W_{1,1} & W_{1,2} & 0 &  W_{2,1} & W_{2,2} & 0 & 0 & 0  \\
%         0       & 0       & 0 & W_{1,2} & 0 & 0 & W_{2,2} & 0 & 0  \\
%         0       & 0       & 0 & W_{1,1} & W_{1,2} & 0 & W_{2,1} & W_{2,2} & 0  \\
%         0       & 0       & 0 & 0 & W_{1,1} & W_{1,2} & 0 & W_{2,1} & W_{2,2}  \\
%     \end{bmatrix}
%     *
%     \begin{bmatrix}
%         x_{1,1} \\
%         x_{1,2} \\
%         x_{1,3} \\
%         x_{2,1} \\
%         x_{2,2} \\
%         x_{2,3} \\
%         x_{3,1} \\
%         x_{3,2} \\
%         x_{3,3} 
%     \end{bmatrix} 
%     % }
% \end{equation}

% \begin{equation}
%     \label{eq-1}
%     y  = Conv(x, W)
% \end{equation}

% \begin{equation}
%     \label{eq-2}
%     y  = M * x
% \end{equation}




% \begin{equation}
%     x = M^{-1}*y
% \end{equation}


% \begin{equation}
%     \scriptsize
%     \label{eq:dy_dw}
%     \frac{\partial x_q}{\partial W_a} = \begin{cases}
%                             0, \textit{  if $a = q$}\\
%                             -\sum_{q' \in (0,0)-(k-1,k-1), q' != (0,0)}{W_{(q'-a)} * \frac{\partial x_{q-q'}}{\partial W_{a}}}  \\ 
%                              \hspace{11em} - x_{q-a}, \hspace{4em} q > a
%                         \end{cases}
% \end{equation}
